Provably Robust Multi-bit Watermarking for AI-generated Text

Large Language Models (LLMs) have demonstrated remarkable capabilities of generating texts resembling human language. However, they can be misused by criminals to create deceptive content, such as fake news and phishing emails, which raises ethical concerns. Watermarking is a key technique to address these concerns, which embeds a message (e.g., a bit string) into a text generated by an LLM. By embedding the user ID (represented as a bit string) into generated texts, we can trace generated texts to the user, known as content source tracing. The major limitation of existing watermarking techniques is that they achieve sub-optimal performance for content source tracing in real-world scenarios. The reason is that they cannot accurately or efficiently extract a long message from a generated text. We aim to address the limitations. In this work, we introduce a new watermarking method for LLM-generated text grounded in pseudo-random segment assignment. We also propose multiple techniques to further enhance the robustness of our watermarking algorithm. We conduct extensive experiments to evaluate our method. Our experimental results show that our method substantially outperforms existing baselines in both accuracy and robustness on benchmark datasets. For instance, when embedding a message of length 20 into a 200-token generated text, our method achieves a match rate of $97.6\%$, while the state-of-the-art work Yoo et al. only achieves $49.2\%$. Additionally, we prove that our watermark can tolerate edits within an edit distance of 17 on average for each paragraph under the same setting.

==> cfp.tex <==
\section{Call for Papers}

The conference seeks submissions presenting novel research results in
all aspects of computer and communications security and privacy,
including both practical and theoretical contributions.

\subsection{Paper Submission Information}

Submissions must be received at \url{https://ccs17.hotcrp.com/} by the
strict deadline of {\bf 19 May 2017 at 8:59 PM PDT (UTC-7)}.
Submitted papers must not substantially overlap with papers that have
been published or that are simultaneously submitted to a journal,
conference, or workshop. Submissions must be anonymized and avoid
obvious self-references.

CCS has traditionally required that authors submitting papers
guarantee that an author will be able to present their paper at the
conference. We recognize, however, that the current travel
restrictions and screening processes may make it impossible or
uncomfortable for some authors to travel to the conference. The venue
for CCS 2017 was selected several years ago, and we do not wish to
exclude any potential authors who may have difficulty traveling due to
recent changes in US immigration practices.  CCS welcomes submissions
by authors of all nationalities, and will make allowances for
presenting papers electronically or with non-author presenters in
cases where paper authors are unable to travel to the United States.

Submissions will be evaluated based on their scientific merit,
novelty, importance, presentation quality, and relevance to computer
and communications security and privacy.  If a paper includes work
that raises ethical concerns it is up to the authors to convince the
reviewers that appropriate practices were followed to minimize
possible harm and that any harm caused by the work is greatly
outweighed by its benefits. The review process will be carried out in
two phases and authors will have an opportunity to provide a
length-limited response to the first-phase reviews.

\subsection{Paper Format}

Submissions must be single PDF files containing at most 12 pages in
the required new ACM format (see
\url{https://www.sigsac.org/ccs2017/format} for details and templates,
which you have presumably found if you are reading this!) of body
content, with any number of additional pages for the bibliography,
well-marked appendices, and any desired supplementary material.  When
relevant, submitters may include reviews from past submissions and
responses to them in the supplementary material.

Reviewers are not required to consider the appendices or supplementary
material, however, so submissions need to be intelligible and
convincing without them.  Submissions not meeting these guidelines, or
playing games to work around page limits, will be rejected by the PC
chairs without review.  In particular, papers should not use squeezing
tricks to adjust the (already very dense) ACM paper format, and moving
discussion of key related work or important definitions to appendices
may be grounds for rejection.

\subsection{Practice Talks}

Following the lead of USENIX Enigma, we want to improve the quality of
the conference and provide a better experience for both presenters and
attendees by holding practice sessions before the conference (see
\url{https://www.sigsac.org/ccs2017/practicefaq}). Presenting authors
of accepted papers are expected to participate in an on-line practice
session approximately three weeks before the conference.

\subsection{Conflicts of Interest}

The conference requires cooperation from both authors and program
committee members to ensure a process that is both fair in practice
and perceived to be fair by everyone. When submitting a paper, authors
are required to identify members of the program committee who may not
be able to provide an unbiased review.  This includes people with
strong personal or professional relationships such as advisor/advisee,
members of the same organization, and close collaborators (for
example, recent or repeated co-authors). In general, this means anyone
who a reasonable person with all the relevant information would
question as an impartial reviewer. The program co-chairs reserve the
right to request a more specific description of a conflict-of-interest
declaration from authors.

Program committee members who have a conflict of interest with a
paper, including program co-chairs, will be excluded from evaluation
and discussion of the paper, but because submissions are anonymous to
reviewers it is important for submitting authors to identify these
conflicts. In the case of a program co-chair, the other co-chairs who
do not have conflicts will be responsible for managing that paper.
Program co-chairs are not permitted to be involved as co-authors in
any submissions.




==> discussion.tex <==
\section{Discussion and Limitation}
\noindent
\textbf{Correctness metric.} In our work we focus on using match rate as our evaluation metric for watermark correctness. Several previous work~\cite{luo2020distortion,yang2022tracing,yoo2023robust,yoo2023advancing} in watermarking adopted another metric, bit accuracy (the ratio of correctly extracted bits). However, in many cases, the gap between match rate and bit accuracy may be large. For example, if we use Yoo et al.~\cite{yoo2023advancing} to embed 20 bits into a 200 length paragraph, it achieves an bit accuracy of $94.7\%$, while only $49\%$ match rate.  Consequently, achieving a high bit accuracy does not automatically guarantee an equally high match rate. In practical applications, where the accuracy of extracted information is paramount, even minor extraction errors are unacceptable. Therefore, employing the match rate as a metric offers a more realistic assessment of performance in real-world scenarios.

\noindent
\textbf{Robustness to paraphrasing attacks.}  
While our watermark has demonstrated effectiveness in countering discrete alternations and copy-paste attacks, it is less effective in defending against paraphrasing attacks, particularly when embedding long bit strings into short paragraphs.  We note that it is still an open challenge to develop watermarking (both zero-bit \& multi-bit \cite{fernandez2023three,pmlr-v202-kirchenbauer23a,yoo2023advancing,zhao2023provable}) robust against paraphrasing because it removes/adds many existing/new tokens from a (watermarked) text. Semantic-based watermark~\cite{ren2023robust,liu2023semantic} is a promising direction to enhance robustness against paraphrasing for zero-bit watermarking. However, how to generalize them to multi-bit setting remains unsolved. We believe it is an interesting future work to develop a multi-bit watermark algorithm optimized for defending against paraphrasing. 
%However, it is worth noting that watermarking long textual content, as opposed to short content, presents a more critical challenge. This is due to its potential application in safeguarding intellectual property rights, particularly within the domain of AI-generated articles and novels.
%Several studies~\cite{kirchenbauer2023reliability,zhao2023provable} have identified the inherent challenges in protecting text watermarks against paraphrasing attacks. 

\noindent
\textbf{Gap between theoretical bound and empirical attack.} Figure~\ref{fig:gap} in Appendix \ref{appendix: experiment result} shows the gap between theoretical bound and different empirical attacks. The gap is caused by multiple reasons. On one hand,  there is a substantial gap between the performance of existing attack and that of a theoretically optimal attack. On the other hand, our derived bound has improvement space. For example, in our derivation we considered the worst case that the attacker always uses "edit" operation and this operation causes maximal change to $\mathsf{COUNT}$ matrix. It is possible to derive a better bound when specifically considering copy-paste attack.  We upper-bounded the LHS of Inequality~\ref{ieq:scale} using its RHS. However, there is a gap between the LHS and the RHS. We will try to improve our bound derivation in future work.

\wenjie{shall we deliver these points?}

%\noindent
%\textbf{Adopting other error-correction code scheme.} In our work, we focus on using BCH error-correction code. There are other families of error-correction codes, including Hamming code~\cite{hamming1950error}, Reed-Solomon code~\cite{reed1960polynomial}, Reed-Muller code~\cite{massey1992deep}. We choose BCH code because it provides a large family of codes with different input length and code rate, making it flexible for embedding different bit length. Many of those BCH codes are the best-known ones under the same input length with the best code rate.  However, Hamming code can only recover 1 bit error for any input length, making the watermark vulnerable when embedding lengthy information. Reed-Solomon code is unsuitable due to its encoding process, which generates relatively large finite field elements (typically 255 bits) as output. Consequently, the resulting watermark does not work for short articles with only hundreds of tokens. Similarly, Reed-Muller code requires the input bit length to be a power of 2,  resulting in waste of many bits when embedding information lengths that do not satisfy this criterion.
